Neural Network-based Control Systems with Application to Flight Control, From Classical Neural Control to Reinforcement Learning

This book provides a comprehensive and systematic exploration of neural network-based intelligent control systems for aerospace applications, bridging foundational theory with practical implementation. It is structured into two primary parts: Part I covers model-based control design, detailing Feedback Error Learning (FEL), pseudocontrol strategies, and neural backstepping for strict-feedback systems, along with practical refinements such as learning rule modifications, composite learning, and discrete-time formulations, all grounded in rigorous Lyapunov stability analysis. Part II introduces model-free control, laying the groundwork for Reinforcement Learning and Approximate Dynamic Programming. Throughout, theoretical concepts are solidified through detailed case studies on quadrotor UAVs, fixed-wing aircraft (GTM), satellites, and hypersonic flight vehicles, complete with performance metrics, parameter sensitivity analyses, and discussions of actuator faults, input constraints, and wind disturbances, making the book an invaluable resource for students and practicing engineers seeking to design, simulate, and analyze intelligent flight control systems.

==> acknowledgement.tex <==
%%%%%%%%%%%%%%%%%%%%%%acknow.tex%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample acknowledgement chapter
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer %%%%%%%%%%%%%%%%%%%%%%%%%%

\extrachap{Acknowledgements}

Use the template \emph{acknow.tex} together with the document class SVMono (monograph-type books) or SVMult (edited books) if you prefer to set your acknowledgement section as a separate chapter instead of including it as last part of your preface.



==> acronym.tex <==
%%%%%%%%%%%%%%%%%%%%%%acronym.tex%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample list of acronyms
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer %%%%%%%%%%%%%%%%%%%%%%%%%%

\extrachap{Acronyms}

%Use the template \emph{acronym.tex} together with the document class SVMono (monograph-type books) or SVMult (edited books) to style your list(s) of abbreviations or symbols.

%Lists of abbreviations\index{acronyms, list of}, symbols\index{symbols, list of} and the like are easily formatted with the help of the Springer-enhanced \verb|description| environment.

\begin{description}%[CABR]
\item[ICS]{Intelligent Control System}
\item[IFCS]{Intelligent Flight Control System}
\item[NN]{Neural Network}
\item[RL]{Reinforcement Learning}
\item[FEL]{Feedback Error Learning}
\item[LoA]{Level of Autonomy}
\item[FTC]{Fault-Tolerant Control}
\item[UAV]{Unmanned Aerial Vehicle}
\item[CM]{Control Mechanism}
\item[IRAC]{Integrated Resilient Aircraft Control}
\item[ELM]{Extreme Learning Machine}
\item[PE]{Persistent Excitation}
\item[HGO]{High Gain Observer}
\item[ADP]{Approximate Dynamic Programming}
\item[HJB]{Hamiltonian-Jacobi-Bellman}
\item[HJI]{Hamilton-Jacobi-Isaacs}
\item[MDP]{Markov Decision Process}
\item[DDPG]{Deep Deterministic Policy Gradient}
\item[TRPO]{Trust Region Policy Optimization}
\item[SAC]{Soft Actor-Critic}
\item[PPO]{Proximal Policy Optimization}
\item[BIBO]{Bounded-Input Bounded-Output}
\item[FOSMD]{First-Order Sliding Mode Differentiator}
\item[RBF]{Radial Basis Function}
\item[MLP]{Multilayer Perceptron}
\item[WNN]{Wavelet Neural Network}
\item[RNN]{Recurrent Neural Network}
\item[ENN]{Elman Neural Network}
\item[BPTT]{Backpropagation Through Time}
\item[LSTM]{Long Short-Term Memory}
\item[RTRL]{Real-Time Recurrent Learning}
\item[ELM]{Extreme Learning Machine}
\item[CNN]{Convolutional Neural Network}
\item[MAE]{Mean Absolute Error}
\item[MAEE]{Mean Absolute Estimation Error}
\item[GTM]{Generic Transport Model}
\item[ZoH]{Zero-order Hold}
\item[MWN]{Mean Weight Norm}
\item[MAV]{Micro Aerial Vehicle}
\item[SISO]{Single-Input Single-Output}
\item[MIMO]{Multiple-Input Multiple-Output}
\item[PID]{Proportional-Integral-Derivative}
\item[HFV]{Hypersonic Flight Vehicle}
\item[VTOL]{Vertical Take-off and Landing}
\item[FPA]{Flight Path Angle}
\item[PSD]{Power Spectral Density}
\item[DSC]{Dynamic Surface Control}
\item[NSV]{Near-Space Vehicle}
\item[FOSMD]{First-Order Sliding Mode Differentiator}
\item[HOSMD]{Higher-Order Sliding Mode Differentiator}
\item[SMC]{Sliding Mode Control}
\item[TSMC]{Terminal Sliding Mode Control}
\item[HONN]{Higher Order Neural Network}
\item[UUB]{Uniformly Ultimately Bounded}
\item[RISE]{Robust Integral of the Signum of the Error}
\end{description}

==> dedication.tex <==

%%%%%%%%%%%%%%%%%%%%%%% dedic.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% sample dedication
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer %%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{dedication}
Use the template \emph{dedic.tex} together with the Springer document class SVMono for monograph-type books or SVMult for contributed volumes to style a quotation or a dedication\index{dedication} at the very beginning of your book
\end{dedication}






==> foreword.tex <==
%%%%%%%%%%%%%%%%%%%%%%foreword.tex%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample foreword
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer %%%%%%%%%%%%%%%%%%%%%%%%%%

\foreword

%% Please have the foreword written here
Use the template \textit{foreword.tex} together with the document class SVMono (monograph-type books) or SVMult (edited books) to style your foreword\index{foreword}. 

The foreword covers introductory remarks preceding the text of a book that are written by a \textit{person other than the author or editor} of the book. If applicable, the foreword precedes the preface which is written by the author or editor of the book.


\vspace{\baselineskip}
\begin{flushright}\noindent
Place, month year\hfill {\it Firstname  Surname}\\
\end{flushright}




==> glossary.tex <==
%%%%%%%%%%%%%%%%%%%%%%acronym.tex%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample list of acronyms
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer %%%%%%%%%%%%%%%%%%%%%%%%%%

\Extrachap{Glossary}


Use the template \emph{glossary.tex} together with the Springer document class SVMono (monograph-type books) or SVMult (edited books) to style your glossary\index{glossary} in the Springer layout.


\runinhead{glossary term} Write here the description of the glossary term. Write here the description of the glossary term. Write here the description of the glossary term.

\runinhead{glossary term} Write here the description of the glossary term. Write here the description of the glossary term. Write here the description of the glossary term.

\runinhead{glossary term} Write here the description of the glossary term. Write here the description of the glossary term. Write here the description of the glossary term.

\runinhead{glossary term} Write here the description of the glossary term. Write here the description of the glossary term. Write here the description of the glossary term.

\runinhead{glossary term} Write here the description of the glossary term. Write here the description of the glossary term. Write here the description of the glossary term.

==> preface.tex <==
%%%%%%%%%%%%%%%%%%%%%%preface.tex%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample preface
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer %%%%%%%%%%%%%%%%%%%%%%%%%%

\preface

%% Please write your preface here
Use the template \emph{preface.tex} together with the document class SVMono (monograph-type books) or SVMult (edited books) to style your preface.

A preface\index{preface} is a book's preliminary statement, usually written by the \textit{author or editor} of a work, which states its origin, scope, purpose, plan, and intended audience, and which sometimes includes afterthoughts and acknowledgments of assistance. 

When written by a person other than the author, it is called a foreword. The preface or foreword is distinct from the introduction, which deals with the subject of the work.

Customarily \textit{acknowledgments} are included as last part of the preface.
 

\vspace{\baselineskip}
\begin{flushright}\noindent
Place(s),\hfill {\it Firstname  Surname}\\
month year\hfill {\it Firstname  Surname}\\
\end{flushright}




==> references.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use



==> solutions.tex <==

\Extrachap{Solutions}

\section*{Problems of Chapter~\ref{intro}}

\begin{sol}{prob1}
The solution\index{problems}\index{solutions} is revealed here.
\end{sol}


\begin{sol}{prob2}
\textbf{Problem Heading}\\
(a) The solution of first part is revealed here.\\
(b) The solution of second part is revealed here.
\end{sol}


